Sub-harmonic Injection Locking in Metronomes

In this paper, we demonstrate sub-harmonic injection locking (SHIL) in mechanical metronomes. To do so, we first formulate metronome's physical compact model, focusing on its nonlinear terms for friction and the escapement mechanism. Then we analyze metronomes using phase-macromodel-based techniques and show that the phase of their oscillation is in fact very immune to periodic perturbation at twice its natural frequency, making SHIL difficult. Guided by the phase-macromodel-based analysis, we are able to modify the escapement mechanism of metronomes such that SHIL can happen more easily. Then we verify the occurrence of SHIL in experiments. To our knowledge, this is the first demonstration of SHIL in metronomes; As such, it provides many valuable insights into the modelling, simulation, analysis and design of nonlinear oscillators. The demonstration is also suitable to use for teaching the subject of injection locking and SHIL.

==> hys.tex <==
\section{\normalfont {\large How to Model Hysteresis Properly}}\seclabel{hys}
To develop our memristor models, we first study how to model $i$--$v$ hysteresis in
two-terminal devices properly.
We show that the $i$--$v$ hysteresis can be modelled with the help of an internal
state variable and an implicit differential equation.
Then with the help of an example, we illustrate how a model with internal
unknowns and implicit equations can be properly written in both Verilog-A and
the ModSpec format.

\subsection{Model Template for Devices with $i$--$v$ Hysteresis}\seclabel{hys_eqn}

The equation of a general two-terminal resistive device can be written as
\begin{equation}\eqnlabel{IV_f}
	i(t) = f(v(t)),
\end{equation}
where $v(t)$ is the voltage across the device, $i(t)$ the current through it.
For example, the function $f(.)$ for a simple linear resistor can be written as
\begin{equation}\eqnlabel{R_f}
	f(v(t)) = \frac{v(t)}{R}.
\end{equation}

For devices with $i$--$v$ hysteresis, $i(t)$ and $v(t)$ cannot have a simple
algebraic mapping like \eqnref{IV_f}.
Instead, we introduce a state variable $s(t)$ into \eqnref{IV_f} and rewrite
the $i$--$v$ relationship as 
\begin{equation}\eqnlabel{IV_f1}
	i(t) = f_1(v(t),~s(t)).
\end{equation}

The dynamics of the internal state variable $s(t)$ is governed by a
differential equation:
\begin{equation}\eqnlabel{sV_f2}
	\frac{d}{dt}s(t) = f_2(v(t),~s(t)).
\end{equation}

The internal state variable $s(t)$ can have several physical meanings.
If we consider the original memristor model proposed by Chua in the 1970s
\cite{chua1971memristor,chua1976memristor}, $s(t)$ can be thought of as the
flux or charge stored in the device.
In the context of metal-insulator-metal-(MIM)-structured RAM devices, \eg,
RRAMs and CBRAMs, $s(t)$ can represent either the length of the conductive
filament/bridge, or the gap between the tip of the filament/bridge to the
opposing electrode.\footnote{For CBRAM devices, the tunnelling gap can also form
in the middle of the conductive bridge instead of on one of its ends
\cite{lin2012IEDM}.} \ignore{
For MRAM devices, $s(t)$ may be the internal magnetization that determines the
resistance of the device.}

In all these scenarios, $s(t)$ has some influence on $i(t)$.
So we cannot directly calculate the current based on the voltage applied to the
device at a single time $t$; $i(t)$ also depends on the value of $s(t)$.
On the other hand, at time $t$, the value of $s(t)$ is determined by the
history of $v(t)$ according to \eqnref{sV_f2}.
Therefore, we can think of the device as having internal ``memory'' of the
history of its input voltage.
If we choose the formula for $f_1$ and $f_2$ in \eqnref{IV_f1} and
\eqnref{sV_f2} properly, as we sweep the voltage, hysteresis in the current
becomes possible.

In the rest of this paper, \eqnref{IV_f1} and \eqnref{sV_f2} serve as a model
template for two-terminal devices with $i$--$v$ hysteresis.
To illustrate its use, we design a device example, namely
``\texttt{hys\_example}'', with functions $f_1$ and $f_2$ defined as follows.

\begin{equation}\eqnlabel{hys_f1}
	f_1(v(t), s(t)) = \frac{v(t)}{R} \cdot (\tanh(s(t)) + 1).
\end{equation}

\begin{equation}\eqnlabel{hys_f2}
	f_2(v(t), s(t)) = \frac{1}{\tau} \left( v(t) - s^3(t) + s(t) \right).
\end{equation}

The choice of $f_1$ is easy to understand.
$\tanh()$ is a monotonically increasing function with range $(-1, 1)$.
We add $1$ to it to make its range positive.
We then incorporate it into $f_1$ as a factor such that $s(t)$ can modulate the
conductance of the device between $0$ and $2/R$.

The choice of $f_2$ determines the dynamics of $s(t)$.
And when $f_2 = 0$, the corresponding ($v$, $s$) pairs will show up as part of
the DC solutions of circuits containing this device.
Therefore, if we plot the values of $f_2$ in a contour plot, such as in
\figref{hys_f2} (a), the curve representing $f_2 = 0$ is especially important.
Through the use of a simple cubic polynomial of $s(t)$ in \eqnref{hys_f2}, we
design the $f_2 = 0$ curve to fold back in the middle, crossing the $v = 0$
axis three times.
In this way, when $v$ is around $0$, there are three possible values $s$ can
settle on, all satisfying $\frac{d}{dt} s(t) = f_2 = 0$.
This multiple stability in state variable $s$ is the foundation of hysteresis
found in the DC sweep on the device.

\figref{hys_f2} (b) illustrates how hysteresis takes place in DC sweeps.
In \figref{hys_f2} (b), we divide the $f_2 = 0$ curve into three parts: curve
\texttt{A} and \texttt{B} have positive slopes while \texttt{C} has a negative
one.
When we sweep $v$ towards the right at a very slow speed to approximate DC
conditions, starting from a negative value left of $V-$, at the beginning,
there is only one possible DC solution of $s$. 
As we increase $v$, the ($v$, $s$) pair will move along curve \texttt{A}, until
\texttt{A} ends when $v$ reaches $V+$.
If $v$ increases slightly beyond $V+$, multiple stability in $s$ disappears.
($v$, $s$) reaches the $f_2 > 0$ region and $s$ will grow until it reaches
the \texttt{B} part of the $f_2 = 0$ curve.
This shows up in the DC solutions as a sudden jump of $s$ towards curve
\texttt{B}.
Similarly, when we sweep $v$ in the other direction starting from the right of
$V+$, the ($v$, $s$) pair will follow curve \texttt{B}, then have a sudden
shift to \texttt{A} at $V-$.
Because $V+ > V-$, hysteresis occurs in $s$ when sweeping $v$, as illustrated
in \figref{hys_f2} (b).
Since $s$ modulates the device's conductance, there will also be hysteresis in
the $i$--$v$ relationship. 

\tnote{Here I am using \figref{hys_f2} (b) instead of subfigures because it
seems more convenient, and it looks all right in the pdf. When using
subfigures, we have to adjust image/font size, alignment, and the (sub)captions
are often redundant. And the figure count increases very fast. Here the
subfigures are generated with inkscape.}

\begin{figure}[htbp]
\centering{
    \epsfig{file=./figures/hys_f2.eps,width=0.9\linewidth}
}
\caption{Contour plot of $f_2$ function in \eqnref{hys_f2} and predicted $s$--$v$
         hysteresis curve based on the sign of $f_2$.
    \figlabel{hys_f2}}
\end{figure}

Note that we are analyzing and predicting hysteresis based on the DC solution curve
defined by $f_2(v,~s) = 0$.
This clarifies a common confusion people have. 
As hysteresis is normally defined as a type of time-dependence between output
and input, people often believe that it has nothing to do with the circuit's or
device's DC properties.
It is true that hysteresis is normally observed in transient analysis.
But from the above discussions, we can see that it is indeed generated by the
multiple stability and the abrupt change in DC solutions.
As mentioned earlier, at a certain time $t$, $s(t)$ can be thought of as
encoding the memory of $v(t)$ from the past.
Its multiple stability reflects the different possible sets of history of
$v(t)$.
And the separation between $V+$ and $V-$ in the DC curves ensures that no
matter at what speed we sweep $v$, there will always be hysteresis in the
$s$--$v$ relationship.

When we sweep $v$ back and forth, curve \texttt{C}, the one with a negative
slope in \figref{hys_f2} (b) never shows up in solutions.
The reason is that, although it also consists of solutions of $f_2 = 0$, 
these solutions are not stable.
If a ($v$, $s$) point on curve \texttt{C} is perturbed to move above
\texttt{C}, whether because of physical noise or numerical error, it falls in
the $f_2 > 0$ region and will continue to grow until it reaches \texttt{B}.
Similarly, if it moves below \texttt{C}, it will decrease to curve \texttt{A}.
Therefore, it won't be observed during voltage sweep, leaving only \texttt{A}
and \texttt{B} to form the $s$--$v$ hysteresis curves.

\subsection{Compact Model in MAPP}\seclabel{hys_MAPP}

With the model equations for \texttt{hys\_example} defined in \eqnref{hys_f1}
and \eqnref{hys_f2}, how do we put them into a compact model so that we can
simulate it in circuits?
To answer this question, in this section, we first discuss our formulation of
the general form of device compact models, namely the ModSpec format
\cite{amsallem2011modspec,WaAaWuYaRoCICC2015MAPP}.
Then we develop the ModSpec model for \texttt{hys\_example} and implement it in MAPP
\cite{MAPPwebsite}.

ModSpec is MAPP's way of specifying device models.
A device model describes the relationship between variables using equations.
Among the variables of interest, some are the device's inputs/outputs; they are
related to the circuit connectivity.
We call them the device's I/Os.
In the context of electrical devices, they are branch voltages and currents.
Among all the I/Os, some may be expressed explicitly using the other variables;
they are the outputs of the model's explicit equations.
Furthermore, a device model can also have non-I/O internal unknowns and
implicit equations.
Taking all these possibilities into consideration, we specify model equations
in the following ModSpec format.
\begin{eqnarray}
   \vec z &=& \frac{d}{dt} \vec q_e(\vec x, \vec y) + \vec f_e(\vec x, \vec y, \vec u),
   \eqnlabel{ModSpec1}\\
   0 &=& \frac{d}{dt} \vec q_i(\vec x, \vec y) + \vec f_i(\vec x, \vec y, \vec u).
   \eqnlabel{ModSpec2}
\end{eqnarray}

Vectors $\vec x$ and $\vec z$ contain the device's I/Os: $\vec z$ comprises
those I/Os that can be expressed explicitly (for \texttt{hys\_example}, it
contains only $i$), while $\vec x$ comprises those that cannot (for
\texttt{hys\_example}, it is $v$).
$\vec y$ contains the model's internal unknowns (for \texttt{hys\_example}, it
is $s$), while $\vec u$ provides a mechanism for specifying time-varying inputs
within the device (\eg, as in independent voltage or current sources).
The functions $\vec q_e$, $\vec f_e$, $\vec q_i$ and $\vec f_i$ define the
differential and algebraic parts of the model's explicit and implicit
equations. 

For \texttt{hys\_example}, we can write its model equations in the ModSpec
format as follows.
\begin{equation}\eqnlabel{hys_ModSpec}
    \begin{split}
	&\vec f_e(\vec x, \vec y, \vec u) = \frac{\vec x}{R} \cdot (\tanh(\vec y)+1),
     \text{~~~} \vec q_e(\vec x, \vec y) = 0, \\
	&\vec f_i(\vec x, \vec y, \vec u) = 
	 \vec x - \vec y^3 + \vec y, \text{~~~} 
     \vec q_i(\vec x, \vec y) = - \tau \cdot \vec y,
    \end{split}
\end{equation}
with $\vec x = [v]$, $\vec y = [s]$, $\vec z = [i]$, $\vec u = []$.

We can enter the model information in \eqnref{hys_ModSpec} into MAPP by
constructing a ModSpec object \texttt{MOD}.
The code in \appref{hys_ModSpec_code} shows how to create this device model for
\texttt{hys\_example} entirely in the \MATLAB{} language.
For more detailed description of the ModSpec format, users can issue the
command ``\texttt{help ModSpec\_concepts}'' in MAPP.

\subsection{Simulation Results}\seclabel{hys_simulation}

In this section, we verify our analysis and prediction of $i$--$v$ hysteresis
in \secref{hys_eqn} by testing the compact models presented in
\secref{hys_MAPP} and in a circuit shown in \figref{vsrc_hys}.

\begin{figure}[htbp]
\centering{
    \epsfig{file=./figures/vsrc_hys.eps,width=0.2\linewidth}
}
\caption{Schematic of the test bench circuit for \texttt{hys\_example}.
The three circuit unknowns are node voltage $e_1$, current $i_1$ and internal
state variable $s$.
    \figlabel{vsrc_hys}}
\end{figure}

\begin{figure}[htbp]
\centering{
    \epsfig{file=./figures/test_hys_sweep.eps,width=0.9\linewidth}
}
\caption{Results from DC sweep and transient simulation in MAPP on the circuit
in \figref{vsrc_hys}, showing hysteresis in both $s$ and $i_1$ when sweeping
the input voltage, in either type of the analyses.
    \figlabel{test_hys_sweep}}
\end{figure}

\figref{test_hys_sweep} shows the results from DC sweep and transient
simulation with input voltage sweeping up and down on the circuit in
\figref{vsrc_hys}.
It confirms that hysteresis takes place in both $i$--$v$ and $s$--$v$
relationships of the device.

\begin{figure}[htbp]
\centering{
    \epsfig{file=./figures/test_hys_homotopy.eps,width=1.0\linewidth}
}
\caption{Results from homotopy analysis in MAPP. \tnote{Identical results can also be
generated by Xyce.} (a) 3-D view of all the DC solutions of the circuit in
\figref{vsrc_hys} with voltage input between $-1${\it V} and $1${\it V}.
(b) top view of all the DC solutions shows the folding in the $i$--$v$
characteristic curve, explaining the $i$--$v$ hysteresis in \figref{test_hys_sweep}.
(c) side view of the DC solutions.
    \figlabel{test_hys_homotopy}}
\end{figure}

In \figref{test_hys_sweep} (b), curve \texttt{C} (defined in \figref{hys_f2}
(b)) with a negative slope never shows up in either forward or backward voltage
DC sweep.
This matches our discussion in \secref{hys_eqn}.
In order to plot this curve and complete the DC solutions, also to get
rid of the abrupt change of solutions in DC sweeps, we can use the homotopy
analysis \cite{RoMeTCAD2006}.
Homotopy analysis can track the DC solution curve in the state space.
\tnote{It is implemented in both MAPP and Xyce.}
Results from homotopy analysis on the circuit in \figref{vsrc_hys} are shown in
\figref{test_hys_homotopy}.
We note that all the circuit's DC solutions indeed form a smooth curve in the
state space.
The side view of the 3-D plot displays curve \texttt{C} we have designed in our
model equation \eqnref{hys_f2}.
The corresponding curve in the top view connects the two discontinuous DC sweep
curves in \figref{test_hys_sweep}; it consists of all the unstable solutions in
the $i$--$v$ relationship.
This curve was previously missing in DC and transient sweep results, and now
displayed by the homotopy analysis.
These results from homotopy analysis provide us with important insights into
the model.
They reveal that there is a single smooth and continuous DC solution curve in
the state space, which is an indicator of the well-posedness of the model.
They also illustrate that it is the folding in the smooth DC solution curve
that has created the discontinuities in DC sweep results.
These insights are important for the proper modelling of hysteresis. 

Moreover, the top view explains the use of internal state $s$ for modelling
hysteresis from another angle.
Without the internal state, it would be difficult if not impossible to write a
single equation describing the $i$--$v$ relationship shown in
\figref{test_hys_homotopy} (b).
With the help of $s$, we can easily choose two simple model equations as
\eqnref{hys_f1} and \eqnref{hys_f2}, and the complex $i$--$v$ relationship
forms naturally.



==> newcommands-colours.tex <==
% various colours
\definecolor{mylightgrey}{rgb}{0.6,0.6,0.6}
\definecolor{mydarkgrey}{rgb}{0.3,0.3,0.3}
\definecolor{mybrown}{rgb}{0.6,0.2,0}
\definecolor{mylightgreen}{rgb}{0,1,0}
\definecolor{mydarkgreen}{rgb}{0,0.5,0}
\definecolor{MyDarkGreen}{rgb}{0.0,0.4,0.0} % This is the color used for comments
\definecolor{myorange}{rgb}{1,0.4,0}
\definecolor{mypurple}{rgb}{0.8,0,0.8}
\definecolor{MyDarkRed}{rgb}{0.4,0.0,0.0} % This is the color used for strings


==> newcommands-eg-ie-etc.tex <==
% eg, ie, etc, wrt, viz newcommands
\newcommand{\eg}{{\it e.g.\/}}
\newcommand{\ie}{{\it i.e.\/}}
\newcommand{\wrt}{{\it wrt}}
\newcommand{\viz}{{\it viz.\/}}
\newcommand{\vs}{{\it vs.\/}}
\newcommand{\aka}{{\it aka\/}}
\newcommand{\apriori}{{\it a priori}}
\newcommand{\etc}{\textit{etc.}}                                                
% etc defined so that there is only a single period after it if it is followed 
% by a period
% see: http://en.wikibooks.org/wiki/TeX/def                                      
% see: http://www.tug.org/pipermail/texhax/2004-July/002449.html                 
% see: http://en.wikibooks.org/wiki/TeX/if                                       
%\ifx \etc \undefined                                                             
%  %\def\myarg{#1}                                                                
%  %\def\myfullstop{.}                                                            
%  %\def\etc{#1}{\textit{etc} arg is ``\myarg'' \ifx\myarg\myfullstop\then.\else.#1\fi\/}
%  \def\etc#1{\textit{etc}\if#1..\else.#1\fi}                                     
%\fi                                                                              
%                        


==> newcommands-for-bibtex.tex <==
\newcommand{\BP}{({\textbf{Best Paper}})} % used in bibliography
\newcommand{\BPnom}{({\textbf{Best Paper Nomination}})} % used in bibliography
\newcommand{\IP}{({\textbf{Invited}})} % used in bibliography
\newcommand{\presenter}[1]{#1} % used in bibliography
\newcommand{\putDOI}[1]{#1}
%\newcommand{\putDOI}[1]{}
\newcommand{\DP}{\textbf{(Distinguished Paper)}}


==> newcommands-highlight-ignore.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% newcommands for ignoring, commenting, annotating, highlighting
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ignore}[1]{}
\let\IGNORE=\ignore
%\newcommand{\comment}[1]{} % conflicts with something predefined
\newcommand{\COMMENT}[1]{}
\newcommand{\jrcomment}[1]{{\color{blue}#1}}
\let\jc=\jrcomment
\newcommand{\redHL}[1]{{\color{red}\bf #1}}
\newcommand{\REDHL}[1]{{\color{red}\bf #1}}
\newcommand{\blueHL}[1]{\textbf{\color{blue}#1}}
\newcommand{\jsugg}[1]{\textit{\color{blue}#1}}
\newcommand{\jpvt}[1]{\textit{\color{red}#1}}
%\newcommand{\jsumm}[1]{{\color{blue}{{\uline{\textit{#1}}}}}}
\newcommand{\jsumm}[1]{\centerline{\color{blue}{{\uline{\textit{#1}}}}\\}}
\newcommand{\jkill}[1]{{\color{blue}\sout{#1}}}
\newcommand{\toputback}[1]{{\blueHL{PUT THIS BACK:} #1}}
\newcommand{\jemph}[1]{\textbf{\uline{#1}}}
\newcommand{\jques}[1]{{\color{blue}#1?}}
\let\jnoteignored=\ignore
	
%\newcommand{\jnote}[1]{\textit{\color{blue}#1}}
\newcommand{\jnote}[1]{{\color{mydarkgreen}\textit{\uline{#1}}}}
\ignore{
    \newcommand{\jnote}[1]{% using fixme
    	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
    	\renewcommand{\fixmelogo}{}%
    	\hspace*{-0.35em}\raisebox{0.7em}[\height][\depth]
                {\\\makebox[0em][l]{\fxnote{\tiny{\color{myred}JR: }
                \textit{\color{mydarkgreen}#1}}}}%
    }
}
\let\jn=\jnote
\newcommand{\TOFIX}[1]{% using fixme
	\renewcommand{\fxnotename}[1]{$\!\!\!$}%
	\renewcommand{\fixmelogo}{}%
	{\fxfatal{\bf\normalsize\textit{\color{myred}#1}}}%
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% END newcommands for ignoring, commenting, ....
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> newcommands-labels-refs.tex <==
% label and ref newcommands
% now mostly deprecated (but redefined and kept for backward compatibility) - move to \cref from the cleveref package
\crefname{algocf}{alg.}{algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{equation}{}{}
\Crefname{equation}{}{}

%DONE: xyzref{} should be able to handle multiple arguments so that you can
%reference multiple figures/equations at the same time -AG
%Now fixed with some package/command CREF.
\newcommand{\corrlabel}[1]{\label{corr:#1}}
\newcommand{\corrref}[1]{Corollary \ref{corr:#1}}
\newcommand{\assref}[1]{Assumption \ref{ass:#1}}
\newcommand{\asslabel}[1]{\label{ass:#1}}
%\newcommand{\eqnref}[1]{(\ref{eq:#1})}
%\newcommand{\eqnlabel}[1]{\label{eq:#1}}
\newcommand{\eqnlabel}[1]{\label{#1}}
\newcommand{\eqnref}[1]{\cref{#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Fig.~\ref{fig:#1}}
\newcommand{\figlabel}[1]{\label{#1}}
\newcommand{\figref}[1]{\cref{#1}}
\newcommand{\chaplabel}[1]{\label{chap:#1}}
\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\secref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\exampleref}[1]{Example~\ref{ex:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\tablabel}[1]{\label{tab:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\thlabel}[1]{\label{th:#1}}
\newcommand{\thref}[1]{Theorem~\ref{th:#1}}
\newcommand{\thmlabel}[1]{\label{thm:#1}}
\newcommand{\thmref}[1]{Theorem \ref{thm:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\lemlabel}[1]{\label{lem:#1}}
\newcommand{\lemref}[1]{Lemma \ref{lem:#1}}
\newcommand{\examplelabel}[1]{\label{ex:#1}}
\newcommand{\labexample}[1]{\label{example:#1}}
\newcommand{\refexample}[1]{Example{ }\ref{example:#1}}
\newcommand{\httpref}[1]{}
\let\el=\eqnlabel
\let\er=\eqnref


==> newcommands-math.tex <==
\newcommand{\ddt}[2]{{\frac{d}{d #2}\left. #1 \right.}}
\newcommand{\ddx}[2]{\frac{\partial{#1}}{\partial{#2}}}
\newcommand{\Ddx}[2]{{\frac{D}{d{#2}}\left[ #1 \right]}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\deq}{=}
\newcommand{\I}{I\left[\right]}
\newcommand{\ELL}[1]{L\left[#1\right]}
\newcommand{\w}{\omega}
\newcommand{\calD}{{\cal D}}
\renewcommand{\jmath}{j}
\newcommand{\Pinvt}{{P(t)}^{-1}}
\newcommand{\halmos}{\hskip\textwidth minus\textwidth \rule{6pt}{6pt}}
\newcommand{\calA}{{\cal A}}
\newcommand{\calAT}{{\cal A}^T}
\newcommand{\calL}{{\cal L}}
\newcommand{\calLadj}{\calL^\dagger}
\newcommand{\calR}{{\cal R}}
\newcommand{\Reals}{\Bbb{R}}
\newcommand{\Real}{\Bbb{R}}
\newcommand{\Safe}{\ensuremath{{\bf S}}}
\newcommand{\Pade}{{Pad\'e}}
\newcommand{\Complexes}{\Bbb{C}}
\newcommand{\HvecqLanc}{\Hvec^{(L)}_q}
\newcommand{\HvecqArn}{\Hvec^{(A)}_q}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\calDT}{{\cal D}^T}
\newcommand{\calCtil}{\tilde{\cal C}}
\newcommand{\calJtil}{\tilde{\cal J}}
\newcommand{\calDtil}{\tilde{\cal D}}
\newcommand{\JstarDphi}{J_{\Delta \phi}^*}
\newcommand{\Jstarphi}{J_{\phi}^*}
\newcommand{\vecbphi}{\vec b_{\phi}}
\newcommand{\vecbext}{\vec b_{\text{ext}}}
\newcommand{\phistarIdeal}{\phi_{\text{ideal}}^*}
\newcommand{\apdx}[1]{\appref{#1}} 
\newcommand{\delbydel}[2]{\ensuremath{\frac{\partial {#1}}{\partial {#2}}}}
\newcommand{\delbydeln}[3]{\ensuremath{\frac{\partial^{{#1}}
{#2}}{\partial{#3}^{{#1}}}}}
\newcommand{\delbydelat}[3]{\ensuremath{\left. \frac{\partial
{#1}}{\partial {#2}} \right|_{{#3}}}}
\newcommand{\dee}{\ensuremath{\mathrm{d}}}
\newcommand{\dbyd}[2]{\ensuremath{\frac{\mathrm{d} {#1}}{\mathrm{d}
{#2}}}}
\newcommand{\dbydn}[3]{\ensuremath{\frac{\mathrm{d}^{{#1}}{#2}}
{\mathrm{d}{#3}^{{#1}}}}}
\newcommand {\dist}[1] {{{\rm dist}\left({#1}\right)}}
\def\Matrix#1{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\textdiag}{{\text{diag}}}
\newcommand{\ihat}{\hat{\imath}}
\newcommand{\jhat}{\hat{\jmath}}
\newcommand{\khat}{\hat{k}}
\newcommand{\del}{\nabla}
\newcommand{\Rxx}{R_{\vec x \vec x}}
\newcommand{\Sxx}{S_{\vec x \vec x}}
\newcommand{\Snn}{S_{\vec n \vec n}}
\newcommand{\vecphi}{\vec \phi}
\newcommand{\Dphi}{\Delta \phi}
\newcommand{\vecDphi}{\vv{\Delta \phi}}
\newcommand{\dphi}{\delta \phi}
\newcommand{\vecdphi}{\vv{\delta \phi}}
\newcommand{\ah}{\alpha_g} % g for group
%\newcommand{\tDagger}{{\tilde t}}
\newcommand{\tDagger}{{t^{\!\dagger}}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\texthyphen}{\text{--}}

%The substack command can be used to produce a multi-line subscripts or superscripts:
%\sum_{\substack{0\le i\le m\\ 0<j<n}} P(i,j) produces a two-line subscript underneath the sum.
%A slightly more general form is the subarray environment which allows you to specify that each line should be left-aligned instead of centered, as here:
% \sum_{\begin{subarray}{l} i\in\Lambda\\ 0<j<n \end{subarray}} P(i,j) 

%\newcommand{\be}[1]{\begin{equation}\eqnlabel{#1}} % now moved to cleveref
\newcommand{\be}[1]{\begin{equation}\label{#1}}
\def\ee{\end{equation}}


==> newcommands-squeeze-spaces.tex <==
%%% tweaklist renewcommands
\newcommand{\modifiedListParamters}{
  \setlength{\topsep}{0pt}%
  \setlength{\itemsep}{-0.1em}
  \setlength{\partopsep}{0em}
  \setlength{\parsep}{0em}
  \setlength{\leftmargin}{1.1em}
  \setlength{\itemindent}{0.0em}
}
\renewcommand{\enumhook}{
  \modifiedListParamters
  \setlength{\itemindent}{0.2em}
}
\renewcommand{\itemhook}{
  \modifiedListParamters
}
\renewcommand{\descripthook}{
  \modifiedListParamters
  \setlength{\itemindent}{-1.0em}
}
%%% end tweaklist renewcommands

\ignore{not usually needed, but the definitions have useful info
		Space saving List environment for enumerations.

	\newcounter{myctr}
	\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
   		{\usecounter{myctr}
   		%\setlength{\topsep}{1mm}\setlength{\itemsep}{0.5mm}
   		\setlength{\topsep}{0.3mm}
   		\setlength{\itemsep}{0mm}
   		\setlength{\parsep}{0.3mm}
   		\setlength{\itemindent}{0mm}
   		\setlength{\partopsep}{0mm}
   		\setlength{\labelwidth}{15mm}
   		\setlength{\leftmargin}{4mm}
   		}
	}{\end{list}}

	\newenvironment{myitemize}{\begin{list}{$\bullet$}
	  \ignore{\setlength{\topsep}{0.8mm}\setlength{\itemsep}{0.25mm}}
	  {\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
	  \setlength{\parsep}{0.1mm}
	  \setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
	  \setlength{\labelwidth}{15mm}
	  \setlength{\leftmargin}{4mm}}
	}{\end{list}}
}

%%%% titlesec: squeezing whitespace between section headings
	\titlespacing{\section}{0pt}{*0.5}{*0.5} % {0pt} is indentation; {*0} is 
                                           % space above; {*0.5} is space below
	\titlespacing{\subsection}{0pt}{*0.3}{*0.3}
	\titlespacing{\subsubsection}{0pt}{*0.1}{*0.1}
%%%% end titlesec

%%%% squeezing whitespace in and around figures
    \floatsep=0.5em % space left between floats.
    \textfloatsep=0.5em % space between last top float or first bottom float and the text.
    \intextsep=0em % space left on top and bottom of an in-text float.
    %\dbltextfloatsep is \textfloatsep for 2 column output.
    %\dblfloatsep is \floatsep for 2 column output.
    \abovecaptionskip=0.2em % space above caption
    \belowcaptionskip=0.2em % space below caption
%%%% END squeezing whitespace in and around figures

\makeatletter
\g@addto@macro\normalsize{%
  \setlength\abovedisplayskip{5pt}
  \setlength\belowdisplayskip{5pt}
  \setlength\abovedisplayshortskip{2pt}
  \setlength\belowdisplayshortskip{2pt}
}
\makeatother

\newcommand{\mycaption}[1]{\caption{\tiny #1}}

% for captions spacing
\captionsetup[table]{font={scriptsize},format=hang,indention=0em}     %% change 1.2 as you like
\captionsetup[figure]{font={scriptsize},format=hang,indention=0em}    %% change as you like
 %% or
 %% \captionsetup{font={stretch=1.2}}  %% this affects both figure and table

% replace Figure x in captions by Fig. x
%\renewcommand{\figurename}{Fig.} % doesn't work.
%but \usepackage[figurename=Fig.]{caption} in packages-headers.tex does work.


%\renewcommand{\baselinestretch}{1.5}
%\setstretch{1.5}


%\def\baselinestretch{0.8593}\large\normalsize - this form works locally?
%\renewcommand{\baselinestretch}{0.94} - this form works only in the preamble
%\renewcommand{\baselinestretch}{0.90}
%\renewcommand{\baselinestretch}{0.5}
%\linespread{0.5} % 0.5 -> 7 lines per inch; 0.9 -> a bit more than 6 lines 
%                 % per vertical inch
% \linespread{0.99}

% baselinestretch fixes for squeezing. See also linespread
%\def\ssp{\def\baselinestretch{0.95645}\large\normalsize} % "single space"
%\def\ssp{\def\baselinestretch{0.905}\large\normalsize} % "single space"
\def\ssp{\def\baselinestretch{1.0}\large\normalsize} % "single space"
\def\dsp{\def\baselinestretch{1.5}\large\normalsize} % "double space"
\ssp

% indent paragraphs less (saves space)
\parindent 	1em
% adjust space between paragraphs (0em can obscure paragraph breaks)
\parskip 0.0em


==> newcommands-thm-env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% theorem-like environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\EndProof{\hfill \quad \vrule width 1ex height 1ex depth 0pt  }
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]
%\newtheorem{illustration}{Illustration}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{notation}{Notation}
\newtheorem{theorem}{Theorem}
\newenvironment{sketch}{\noindent{\bf Sketch of Proof}:}{\halmos}
\newenvironment{conjecture}{\noindent{\bf Conjecture}: \em}{}
\newcommand{\numberedtheorem}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thetheorem
		\renewcommand{\thetheorem}{#1}
	}
	\begin{theorem}
	\ifthen{\not\equal{#2}{}}{
		\thmlabel{#2}
	}
	#3
	\end{theorem}
	\ifthen{\not\equal{#1}{}}{
		\let\thetheorem=\oof
		\addtocounter{theorem}{-1}
	}
}
\newcommand{\numberedlemma}[3]{
	\ifthen{\not\equal{#1}{}}{
		\let\oof=\thelemma
		\renewcommand{\thelemma}{#1}
	}
	\begin{lemma}
	\ifthen{\not\equal{#2}{}}{
		\lemlabel{#2}
	}
	#3
	\end{lemma}
	\ifthen{\not\equal{#1}{}}{
		\let\thelemma=\oof
		\addtocounter{lemma}{-1}
	}
}


==> packages-headers.tex <==
%%%%%%%%%%%%%%%%%% PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%
\RequirePackage{times}
%\RequirePackage[usenames]{pstcol} 
\RequirePackage[usenames]{pstricks} 

% Graphics (figures/images etc.)
%\usepackage[pdftex]{graphicx}
\RequirePackage{graphicx} % supplies \includegraphics
\graphicspath{{./figures/}{./snapshots/}}
\DeclareGraphicsExtensions{.eps,.pdf,.jpeg,.png}

\RequirePackage{rotating}
\RequirePackage{indentfirst} 
\RequirePackage{color} 
%\RequirePackage{picins} 
\RequirePackage{bmpsize} 
\RequirePackage{epsfig} % good old way of including figures
\RequirePackage{eepic} 
\RequirePackage{subfigure} % put figures side-by-side
\RequirePackage{wrapfig} % wrap text around figures
\RequirePackage{picinpar} % alternative to wrapfig, less useful

% Math (symbols/equations etc.)
\usepackage{cancel}
\RequirePackage{amsmath,amssymb,amsthm,amsbsy,amsfonts,dotlessj} 
\RequirePackage{latexsym}
\RequirePackage{mathptm} % - AG (Don't like \mathcal{C} that this produces
\RequirePackage{mathptmx} % times (smaller) math fonts, greek characters also italicized
\RequirePackage{bm} % boldmath
\DeclareMathVersion{bold} 

% Formatting
\RequirePackage{multicol}
\RequirePackage{esvect} % defines \vv{}
\RequirePackage{ifthen}
\RequirePackage{etoolbox}
\RequirePackage{relsize}
\RequirePackage{soul}   % Provides \hl{some-text}
%\RequirePackage{showkeys} 
%\RequirePackage[final,notref]{showkeys} 
%\RequirePackage[top=0.8cm,bottom=0.8cm,left=0.8cm,right=0.8cm,nohead,nofoot]{geometry}
%\RequirePackage[top=1.2cm,bottom=1.3cm,left=1.2cm,right=1.2cm,nohead,nofoot]{geometry}

\usepackage[nolist,nohyperlinks]{acronym}
\RequirePackage{setspace}
\RequirePackage{moreverb}
\RequirePackage{ulem} % provides \uline
        \let\em=\it % ulem package redefines \em=\uline
\RequirePackage[sectionbib]{chapterbib}
\RequirePackage{fancyhdr}
\RequirePackage{array}
\RequirePackage{floatflt} % does (to some extent) work inside itemize environment %
                          % use \fltditem, see $LATEXDOCS/floatflt.pdf, esp. Sec 3.1
\RequirePackage{srcltx}
\RequirePackage{chemarrow}

% Utilities
\RequirePackage{tcolorbox}
\RequirePackage{fixme}
\RequirePackage[footnotesize,bf,figurename=Fig.,hang]{caption}
%\usepackage[scriptsize,hang,bf]{caption}
%\RequirePackage[hypertex]{hyperref} 
\RequirePackage{hyperref} 
%\definecolor{linkColor}{rgb}{0.1,0.1,0.8}
%\usepackage[colorlinks=true,bookmarks,pdfpagemode=UseOutlines,linkcolor=linkColor,citecolor=linkColor,pagecolor=blue,urlcolor=blue,pdftitle={Verification, Learning, Control},pdfauthor={Jaijeet Roychowdhury},plainpages=false]{hyperref}

\usepackage{./tweaklist} % allow changing of item spacings in standard itemize,
                         % enumerate, description environments
					     %%% tweaklist: compress lists. Also check out 
                         %%% \usepackage{mdwlist} (use itemize*, enumerate*, 
                         %%% description* with that)
                         % enumhook for the enumerate environment, itemhook for
                         % the itemize environment, and descripthook for the
                         % description environment.

\providecommand{\subparagraph}{} % needed for IEEEtran.cls (which does not define subparagraph); \providecommand checks if it is already defined
\RequirePackage[small,compact]{titlesec} % squeezing whitespace between section heading
\RequirePackage[square,sort&compress,numbers]{natbib} % needed for IEEEtran; but proposal.cls pulls it in automatically
%\RequirePackage{cite} % natbib doesn't like this
\RequirePackage{lipsum}
\RequirePackage{microtype}
\RequirePackage{url}
\RequirePackage{listings} % Required for insertion of code
\RequirePackage{multirow}
\RequirePackage{booktabs}
% load cleveref last, but before algorithm2e (which breaks cleveref)
\RequirePackage[compress,capitalise,noabbrev]{cleveref} % defines \cref, \Cref, etc; options are compress (don't sort), sort (don't compress), sort&compress (default), nosort (neither sort nor compress)
%\RequirePackage{algorithmic}
%\RequirePackage{algorithm}
%\RequirePackage[boxed,algoruled]{algorithm2e}
\RequirePackage[boxed,algoruled,linesnumbered,vlined,nofillcomment]{algorithm2e}

%%%%%%%%%%%%%%%%%% END PACKAGE INCLUDES %%%%%%%%%%%%%%%%%%%

% fixme package setup
\fxsetup{ status=draft,
		  %author={\tiny JR},
	  	  layout=footnote,
		  layout=inline, % also try footnote or pdfnote
		  theme=color,
	  	  marginclue
}
\definecolor{mydarkgreen}{rgb}{0.0,0.5,0.0}
\definecolor{myred}{rgb}{0.9,0.0,0.0}
%\definecolor{fxnote}{rgb}{0.8000,0.0000,0.0000}
\renewcommand{\englishlistfixmename}{List of changes needed}
% Decrease spacing between items in bib
\newcommand{\BIBdecl}{\setlength{\itemsep}{0.25 em}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Multi-column the bib
%\patchcmd{\thebibliography}
%  {\list}
%  {\begin{multicols}{2}\list}
%    {}
%    {}
%\appto{\endthebibliography}{\end{multicols}}

%------------------------------------------------------------------------------
%   CODE INCLUSION CONFIGURATION
%------------------------------------------------------------------------------

\lstloadlanguages{Matlab}
\lstset{language=Matlab,
        frame=single, % Single frame around code
        basicstyle=\scriptsize\ttfamily,
        % keywordstyle=[1]\color{blue}\bf, % Perl functions bold and blue
        keywordstyle=[3]\color{blue}\underbar, % Custom functions underlined and blue
        identifierstyle=, % Nothing special about identifiers                                         
        commentstyle=\usefont{T1}{pcr}{m}{sl}\color{MyDarkGreen}\scriptsize, 
            % Comments are in small dark green courier font
        stringstyle=\color{MyDarkRed}, 
        showstringspaces=false, % Don't put marks in string spaces
        tabsize=4, % 5 spaces per tab
        % 
        % Put standard functions not included in the default language here
        %morekeywords={rand},
        % Put function parameters here
        %morekeywords=[2]{on, off, interp},
        % Put user defined functions here
        %morekeywords=[3]{test},
        %
        morecomment=[l][\color{blue}]{...}, % Line continuation (...) like blue comment
        % numbers=left, % Line numbers on left
        % firstnumber=1, % Line numbers start with line 1
        % numberstyle=\tiny\color{blue}, % Line numbers are blue and small
        % stepnumber=5 % Line numbers go in steps of 5
}

% Creates a new command to include an Matlab script, the first parameter is the
% filename of the script (without .pl), the second parameter is the caption
\newcommand{\matlabscript}[2]{
    \begin{itemize}
    \item[]\lstinputlisting[caption=#2,label=#1]{#1}
    \end{itemize}
}


\input newcommands-colours
\input newcommands-highlight-ignore
\input newcommands-eg-ie-etc
\input newcommands-labels-refs
\input newcommands-math
\input newcommands-thm-env
\input newcommands-for-bibtex
\input newcommands-squeeze-spaces

